SENTAUR: Security EnhaNced Trojan Assessment Using LLMs Against Undesirable Revisions

A globally distributed IC supply chain brings risks due to untrusted third parties. The risks span inadvertent use of hardware Trojan (HT), inserted Intellectual Property (3P-IP) or Electronic Design Automation (EDA) flows. HT can introduce stealthy HT behavior, prevent an IC work as intended, or leak sensitive data via side channels. To counter HTs, rapidly examining HT scenarios is a key requirement. While Trust-Hub benchmarks are a good starting point to assess defenses, they encompass a small subset of manually created HTs within the expanse of HT designs. Further, the HTs may disappear during synthesis. We propose a large language model (LLM) framework SENTAUR to generate a suite of legitimate HTs for a Register Transfer Level (RTL) design by learning its specifications, descriptions, and natural language descriptions of HT effects. Existing tools and benchmarks are limited; they need a learning period to construct an ML model to mimic the threat model and are difficult to reproduce. SENTAUR can swiftly produce HT instances by leveraging LLMs without any learning period and sanitizing the HTs facilitating their rapid assessment. Evaluation of SENTAUR involved generating effective, synthesizable, and practical HTs from TrustHub and elsewhere, investigating impacts of payloads/triggers at the RTL. While our evaluation focused on HT insertion, SENTAUR can generalize to automatically transform an RTL code to have defined functional modifications.

==> files/background.tex <==
\section{Background}\label{sec:2}
\subsection{Large Language Models (LLMs)}
LLMs refer to advanced AI models, like OpenAI's GPT (Generative Pre-trained Transformer) series, that are trained on vast amounts of text data to understand, generate, and process human-like language patterns and information. LLMs use deep learning architectures and are capable of performing various natural language processing tasks such as text completion, language translation, summarization, and question-answering, among others. These models are designed to comprehend and generate human-like text based on the patterns and information they've learned during training.

 GPT-4 demonstrates an advanced ability to understand and generate human-like text across various languages, providing coherent and contextually relevant responses to prompts. It is one of the largest language models, comprising 175 billion parameters, allowing for a vast understanding of diverse language patterns and information. The model can adapt to different tasks and domains with minimal fine-tuning, making it versatile for various applications, including language translation, text summarization, question-answering, and more.
\subsection{Hardware Trojans}
Hardware Trojans are intentional alterations in designs that introduce undesired functionalities beyond specified requirements. 
Trojans can infiltrate various design abstractions throughout its lifecycle, such as soft IP (e.g., RTL), firm IP, gate-level netlist, or within the IC by an untrusted foundry. These malicious functions can encompass leaking information, operational malfunctioning during crucial activities, or circumventing security protocols. Fundamentally, Trojans comprise trigger and payload sub-circuits. The trigger activates the Trojan under specific conditions to evade detection, often using improbable activation sequences derived from input signals in the design. Payloads execute malicious functions through functional output, side-channel effects, or parametric values (e.g., temperature, current).
